Search by a Metamorphic Robotic System in a Finite 3D Cubic Grid

We consider search in a finite 3D cubic grid by a metamorphic robotic system (MRS), that consists of anonymous modules. A module can perform a sliding and rotation while the whole modules keep connectivity. As the number of modules increases, the variety of actions that the MRS can perform increases. The search problem requires the MRS to find a target in a given finite field. Doi et al. (SSS 2018) demonstrate a necessary and sufficient number of modules for search in a finite 2D square grid. We consider search in a finite 3D cubic grid and investigate the effect of common knowledge. We consider three different settings. First, we show that three modules are necessary and sufficient when all modules are equipped with a common compass, i.e., they agree on the direction and orientation of the $x$, $y$, and $z$ axes. Second, we show that four modules are necessary and sufficient when all modules agree on the direction and orientation of the vertical axis. Finally, we show that five modules are necessary and sufficient when all modules are not equipped with a common compass. Our results show that the shapes of the MRS in the 3D cubic grid have richer structure than those in the 2D square grid.

==> introduction.tex <==
\section{Introduction}
\label{intro}

Swarm intelligence has shed light to collective behavior of 
autonomous entities with simple rules, 
such as ant, boid, and particles. 
The notion is applied to a collection of robots and 
swarm robotics has attracted much attention in the past two decades. 
Each autonomous element of the system is called 
a robot, module, agent, process, and sensor, 
and a variety of swarm robot systems have been investigated  
such as the \emph{autonomous mobile robot system}~\cite{SY99}, 
the \emph{population protocol model}~\cite{AADFP04}, 
the \emph{programmable particles}~\cite{DDGRSS14}, 
\emph{Kilobot}~\cite{RCN14}, 
and \emph{3D Catoms}~\cite{TPB19}. 
Dumitrescu et al. considered the \emph{metamorphic robotic system} (MRS), 
that consists of a collection of \emph{modules} in the infinite 2D square grid~\cite{DSY04a,DSY04b}. 
The modules are \emph{anonymous}, i.e., they are indistinguishable. 
They are \emph{autonomous} and \emph{uniform}, i.e., 
each module autonomously decides its movement by a common algorithm. 
They are \emph{oblivious}, i.e., each module has no memory of past. 
Thus, each module decides its behavior by 
observing other modules in nearby cells. 
Each module can perform a \emph{sliding} to a side-adjacent cell 
and a \emph{rotation} by $90$ degrees around a cell. 
The modules must keep \emph{connectivity}, which is defined by 
side-adjacency of cells occupied by modules. 
The authors considered \emph{reconfiguration} of the MRS, 
that requires the MRS to change the initial shape 
to a specified final shape~\cite{DSY04a}. 
They showed that any horizontally convex connected initial shape of an MRS 
can be transformed to any convex final shape via a straight chain shape. 
Later Dumitrescu and Pach showed that any connected initial shape 
can be transformed to any connected final shape via a 
straight chain shape~\cite{DP06}. 
In other words, the MRS has the ability of "universal reconfiguration." 
% These results also reveal the structure of the state transition graph of the MRS.

Reconfiguration can generate dynamic behavior of the MRS. 
Dumitrescu et al. demonstrated that the MRS can move forward 
by repeating a reconfiguration~\cite{DSY04b}. 
They showed a reconfiguration that realizes the fastest \emph{locomotion}. 
Doi et al. pointed out that the oblivious modules can use the 
shape of the MRS as global memory and 
the MRS can solve more complicated problem 
as the number of modules increases. 
They investigated \emph{search} in a finite 2D square grid, 
that requires the MRS to find a target cell in a finite 
rectangle \emph{field}~\cite{DYKY18}. 
Each module does not know the position of the target cell or   
the initial configuration % position or the initial shape 
of the MRS. 
They showed that the MRS can find the target cell 
by sweeping each row of the field without such a priori knowledge. 
Specifically, if the modules agree on the cardinal directions 
(i.e., north, south, east and west), 
three modules are necessary and sufficient, 
otherwise five modules are necessary and sufficient. 
Nakamura et al. considered \emph{evacuation} of the MRS from a 
finite rectangular field in the 2D square grid~\cite{NSY20}. 
There is a hole (i.e., two side-adjacent cells) 
on the wall of the field, 
and the MRS is required to exit from it from an arbitrary 
initial position and arbitrary initial shape. 
They showed that two modules are necessary and sufficient 
when the modules agree on the cardinal directions, 
otherwise four modules are necessary and sufficient. 

In this paper, we investigate the effect of common knowledge 
on search by the MRS in the 3D cubic grid. 
We consider the following three cases: 
$(i)$ modules equipped with a common \emph{compass} 
(i.e., they agree on the direction and orientation of $x$, $y$, and $z$ axes).
$(ii)$ modules equipped with a common vertical axes 
(i.e., they agree on the direction and orientation of $z$ axes), 
and 
$(iii)$ modules not equipped with a common compass 
(i.e., they have no agreement on directions and orientations). 
We demonstrate that 
three modules are necessary and sufficient when 
the modules are equipped with a common compass 
and five modules are necessary and sufficient 
when the modules are not equipped with a common compass. 
The numbers of sufficient modules in the 3D cubic grid 
are the same as those in the 2D square grid~\cite{DYKY18} 
because the MRS has more states in the 3D cubic grid 
than in the 2D square grid. 
% and three and five modules are sufficient to 
% generate and remember its move. 
For the intermediate case with a common vertical axis, 
we demonstrate that four modules are necessary and sufficient. 
Thus, our results in the 3D cubic grid 
show a smooth trade-off between 
the computational power of the MRS and 
common knowledge among modules, that the previous results 
in the 2D square grid could not find.  
We present search algorithms for these three settings 
and 
show the necessity by examining the 
state transition graph of the MRS. 

\noindent{\bf Related work.}~Reconfiguration of swarm robot systems 
have been discussed for the MRS~\cite{DP06,DSY04a}, 
autonomous mobile robots~\cite{FYOKY15,SY99} and 
the programmable particles~\cite{DGRSS15,DFSVY20}. 
Michail et al. considered the \emph{programmable matter system},
that is similar to the MRS
and investigated reconfiguration by rotations only and 
that by rotations and slidings~\cite{MSS19}. 
They showed that the combination of rotations and slidings 
guarantees universal reconfiguration, 
while rotations only cannot. 
They also presented $\Order(n^2)$-time reconfiguration algorithm 
by rotations and slidings. 
Almethen et al. considered reconfiguration by \emph{line-pushing}, 
where each module is equipped with the ability of pushing a line of 
modules~\cite{AMP20a}. 
They presented $\Order(n \log n)$-time universal reconfiguration algorithm 
that does not promise connectivity of intermediate shapes 
and $\Order(n \sqrt{n})$-time reconfiguration algorithm 
that transforms a diagonal line into a straight chain with 
preserving connectivity. 
The same authors later showed that their programmable matter system 
has the ability of universal reconfiguration 
and $\Order(n \sqrt{n})$-time reconfiguration algorithm 
together with $\Omega(n \log n)$ lower bound~\cite{AMP20b}. 

